PAWS: A Tool for the Analysis of Weighted Systems

PAWS is a tool to analyse the behaviour of weighted automata and conditional transition systems. At its core PAWS is based on a generic implementation of algorithms for checking language equivalence in weighted automata and bisimulation in conditional transition systems. This architecture allows for the use of arbitrary user-defined semirings. New semirings can be generated during run-time and the user can rely on numerous automatisation techniques to create new semiring structures for PAWS' algorithms. Basic semirings such as distributive complete lattices and fields of fractions can be defined by specifying few parameters, more exotic semirings can be generated from other semirings or defined from scratch using a built-in semiring generator. In the most general case, users can define new semirings by programming (in C#) the base operations of the semiring and a procedure to solve linear equations and use their newly generated semiring in the analysis tools that PAWS offers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{75}
\providecommand{\publicationstatus}{De Vink and Wiklicky (Eds.): QAPL 2017\\
EPTCS 250, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.250.5}{10.4204/EPTCS.250.5}}
\pdfoutput=1

